Visibility Reasoning for Concurrent Snapshot Algorithms

Visibility relations have been proposed by Henzinger et al. as an abstraction for proving linearizability of concurrent algorithms that obtains modular and reusable proofs. This is in contrast to the customary approach based on exhibiting the algorithm's linearization points. In this paper we apply visibility relations to develop modular proofs for three elegant concurrent snapshot algorithms of Jayanti. The proofs are divided by signatures into components of increasing level of abstraction; the components at higher abstraction levels are shared, i.e., they apply to all three algorithms simultaneously. Importantly, the interface properties mathematically capture Jayanti's original intuitions that have previously been given only informally.

==> macros.tex <==


\makeatletter
\renewcommand{\ALG@beginalgorithmic}{\small}
\makeatother
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}%


\newcommand{\sigSpacing}{1.1} %

\newcommand{\eqSpacing}{1.1} %

\newcommand{\sepAfterVar}{0.5mm}
\newcommand{\sepAfterBox}{1mm}
\newcommand{\sepInnerProp}{0.8em}
\newcommand{\sepLastProp}{0.1mm}
\newcommand{\sepEvSig}{1.5mm}


\def\useanchorwidth{T}
\stackMath

\makeatletter
\newcounter{algorithmicH}%
\let\oldalgorithmic\algorithmic
\renewcommand{\algorithmic}{%
  \stepcounter{algorithmicH}%
  \oldalgorithmic}%
\renewcommand{\theHALG@line}{ALG@line.\thealgorithmicH.\arabic{ALG@line}}
\makeatother

\DeclareFontFamily{U}{stmry}{}
\DeclareFontShape{U}{stmry}{m}{n}
 {
  <-5.5>  stmary5
  <5.5-6.5> stmary6
  <6.5-7.5> stmary7
  <7.5-8.5> stmary8
  <8.5-9.5> stmary9
  <9.5->  stmary10
   }{}

\usetikzlibrary{arrows,arrows.meta,positioning,shapes,decorations.pathreplacing}

\newcolumntype{A}{ >{$} r <{$} @{} >{${}} l <{$} }

\numberwithin{equation}{subsection}

\algrenewcommand\textproc{}

\algnewcommand\algorithmicresource{\quad\textbf{resource}}
\algnewcommand\Resource{\item[\algorithmicresource]}

\crefname{ax}{Axiom}{Axioms}
\creflabelformat{ax}{\textnormal{(#2#1#3)}}
\crefname{prop}{Property}{Properties}
\creflabelformat{prop}{\textnormal{(#2#1#3)}}


\newcounter{subeq}
\renewcommand{\thesubeq}{\theequation\alph{subeq}}
\newcommand{\newsubeqblock}{%
  \setcounter{subeq}{0}%
  \stepcounter{resetsubeq}%
  \refstepcounter{equation}%
}
\newcommand{\mysubeq}{\refstepcounter{subeq}\tag{\thesubeq}}
\newcommand{\insertSubeq}{\refstepcounter{subeq} (\thesubeq)}

\newcounter{resetequation}
\newcounter{resetsubeq}
\makeatletter
\@addtoreset{equation}{resetequation}
\@addtoreset{subeq}{resetsubeq}
\makeatother

\newcommand{\insertEq}{\refstepcounter{equation} (\theequation)}
\newcommand{\axiomset}[1]{%
  \setcounter{equation}{0}%
  \stepcounter{resetequation}%
  \gdef\theequation{\mbox{#1.\arabic{equation}}}%
}
\newcommand{\mytag}[1]{%
  \setcounter{equation}{0}%
  \stepcounter{resetequation}%
  \gdef\theequation{\mbox{#1}}%
}

\newtheorem*{nonamethm}{\nonamethmname}
\newcommand{\nonamethmname}{}

\newenvironment{genthm}[1]
 {\renewcommand{\nonamethmname}{#1}\nonamethm}
 {\endnonamethm}
\newenvironment{genthm*}[1]
 {\renewcommand{\nonamethmname}{#1}\nonamethmcheck}
 {\endnonamethm}

\newcommand\nonamethmcheck[1][]{%
  \if\relax\detokenize{#1}\relax
    \nonamethm\relax
  \else
    \nonamethm[#1]%
  \fi
  \mbox{}%
}

\newcommand{\mute}[1]{\ifdraft{#1} \else{} \fi}

\newcounter{ToDos}
\newcounter{WarnCounts}

\newcommand{\decorateWC}{
  \stepcounter{WarnCounts}
  \checkoddpage
  \ifoddpageoroneside
     \mbox{}\marginnote{\textcolor{red}{$\skull_{\theWarnCounts}$}}
     \else
     \reversemarginpar
     \mbox{}\marginnote{\textcolor{red}{$\skull_{\theWarnCounts}$}}
     \normalmarginpar
   \fi
}

\newcommand{\signedComment}[3]
           {\mute{\decorateWC\textcolor{#2}{(#1: {#3})}}}

\newcommand{\an}[1]{\signedComment{Aleks}{red}{#1}}
\newcommand{\jo}[1]{\signedComment{Joakim}{red}{#1}}


\newcommand{\rom}[1]{\lowercase\expandafter{\romannumeral #1\relax}}

\definecolor{lightergray}{gray}{0.85}
\definecolor{darkgreen}{rgb}{0,0.4,0}
\definecolor{darkblue}{rgb}{0,0,0.6}

\colorlet{rep}{darkblue}
\colorlet{abs}{magenta}
\colorlet{vrt}{darkgreen}
\newcommand{\repColorName}{\textcolor{rep}{blue}}
\newcommand{\absColorName}{\textcolor{abs}{magenta}}
\newcommand{\vrtColorName}{\textcolor{vrt}{green}}
\newcommand{\rep}[1]{{\color{rep}#1}}%
\newcommand{\abs}[1]{{\color{abs}#1}}%
\newcommand{\vrt}[1]{{\color{vrt}#1}}%

\newcommand{\WrSetDesc} {Set of all writes of cell $i$ of the snapshot
  in history}
\newcommand{\ScSetDesc} {Set of all scans of the snapshot in history}
\newcommand{\VscSetDesc}{Set of virtual scans}
\newcommand{\ScVscDesc} {Partial mapping of abs scans into virtual scans}

\newcommand{\signatureHeader}[2]{%
  \begin{tabular*}{0.9\textwidth}{l@{\extracolsep{\fill}}r}
  \toprule
  \signature{#1} & \textbf{#2}\\
  \midrule
\end{tabular*}%
}

\newenvironment{letbox}[1]{%
\begin{tabular*}{0.9\textwidth}{|@{\hskip 0.2em}l#1@{\extracolsep{\fill}}r|}%
  \hline%
  \textbf{Let}%
  }{%
  \hline%
\end{tabular*}\vspace{\sepAfterBox}%
}

\DeclareRobustCommand{\hlgray}[1]{{\sethlcolor{lightergray}\hl{#1}}}
\DeclareRobustCommand{\hlgreen}[1]{{\sethlcolor{green}\hl{#1}}}
\newcommand{\texttag}[2]{\hlgray{\textsuperscript{(\rom{#1})}#2}}

\newcommand{\mathcolorbox}[2]{\colorbox{#1}{$\displaystyle #2$}}
\newcommand{\mathhl}[1]{\mathcolorbox{lightergray}{#1}}

\newcommand{\signature}[1]{\textbf{signature}\ \ #1\ \ $\defeq$}
\newcommand{\evsignature}[1]{\textbf{event signature}\ \ #1\ \ $\defeq$}
\newcommand{\bigProd}{\mathrlap{\scaleobj{1.2}{\prod}}{\hskip 1.5em}}
\newcommand{\bigSum}{\mathrlap{\scaleobj{1.2}{\sum}}{\hskip 1.5em}}
\newcommand{\bigExists}{\raisebox{-2pt}[0pt][0pt]{\ensuremath{\scaleobj{1.5}{\exists}}}}

\newcommand{\defeq}{\triangleq}
\newcommand{\set}{\vcentcolon=}


\newcommand{\fun}{\to}
\newcommand{\parfun}{\rightharpoonup}

\newcommand{\wideSymbol}[1]{\mathrlap{\ \ #1}\hphantom{{} \subseteq {}}}
\newcommand{\widerSymbol}[1]{\mathrlap{\quad #1}\hphantom{{} \implies {}}}

\newcommand{\wideColon}{\wideSymbol{:}}
\newcommand{\wideEq}{\wideSymbol{\!=}}
\newcommand{\wideDefeq}{\widerSymbol{\defeq}}
\newcommand{\wideIn}{\widerSymbol{\in}}
\newcommand{\wideNi}{\widerSymbol{\ni}}

\newcommand{\relrightarrow}[1]{%
  \mathrel{\raisebox{-2pt}{\protect{\ensuremath{\xrightarrow{\protect{\raisebox{-2pt}[0pt][0pt]{\ensuremath{\scriptstyle{#1}}}}}}}}}%
}
\newcommand{\reflrelrightarrow}[1]{%
  \mathrel{\raisebox{-2pt}{\protect{\ensuremath{\xRightarrow{\protect{\raisebox{-2pt}[0pt][0pt]{\ensuremath{\scriptstyle{#1}}}}}}}}}%
}

\newcommand{\rb}{\sqsubset}
\newcommand{\rbeq}{\sqsubseteq}
\newcommand{\obs}{\prec}
\newcommand{\obseq}{\preccurlyeq}
\newcommand{\hb}{\vartriangleleft}
\newcommand{\hbeq}{\trianglelefteqslant}
\newcommand{\ha}{\vartriangleright}
\newcommand{\haeq}{\trianglerighteqslant}
\newcommand{\robs}{\relrightarrow{\mathbf{rf}}}
\newcommand{\robseq}{\reflrelrightarrow{\mathbf{rf}}}
\newcommand{\hlrobs}{\relrightarrow{\mathhl{\scriptstyle\mathbf{rf}}}}
\newcommand{\wobs}{\relrightarrow{\mathbf{wr}}}
\newcommand{\hlwobs}{\relrightarrow{\mathhl{\scriptstyle\mathbf{wr}}}}
\newcommand{\sobs}{\relrightarrow{\mathbf{sc}}}
\newcommand{\fobs}{\relrightarrow{\mathbf{fwd}}}
\newcommand{\llobs}{\relrightarrow{\mathbf{ll}}}
\newcommand{\rbhbeqrobs}{\rb\hbeq\robs}
\newcommand{\whb}{\hb_w}
\newcommand{\whbS}{\hb_{w1}}
\newcommand{\whbI}{\relrightarrow{\mathbf{wrDiff}}}
\newcommand{\wlt}{<_w}

\newcommand{\subev}{\subseteq}


\newcommand{\term}{\mathcal{T}}


\newcommand{\miniskip}{\par\vskip1mm}
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}

\renewcommand{\Procedure}[3]{%
  \State%
  \underline{%
    \textproc{#1}%
    \ifthenelse{\equal{#2}{}}{}{(#2)}%
    \ifthenelse{\equal{#3}{}}{}{$:$ #3}%
    \ \ $\defeq$%
  }%
}
\renewcommand{\EndProcedure}{}

\newcommand{\writeProc}{\textsc{write}}
\newcommand{\readProc}{\textsc{read}}
\newcommand{\scanProc}{\textsc{scan}}
\newcommand{\vscanProc}{\textsc{vscan}}
\newcommand{\forwardProc}{\textsc{forward}}
\newcommand{\pushLSProc}{\textsc{pushVS}}

\newcommand{\aregSig}{\mathsf{AReg}}
\newcommand{\llregSig}{\mathsf{LLReg}}
\newcommand{\snapshotSig}{\mathsf{Snapshot}}
\newcommand{\fwdSig}{\mathsf{Forwarding}}
\newcommand{\mwFwdSig}{\mathsf{MWForwarding}}

\newcommand{\getpid}{\mathsf{get}\PID}

\newcommand{\writer}{\mathbf{W}}
\newcommand{\reader}{\mathbf{R}}
\newcommand{\LLins}{\mathbf{LL}}
\newcommand{\SCins}{\mathbf{SC}}
\newcommand{\VLins}{\mathbf{VL}}
\newcommand{\LLop}{\textsc{LL}}
\newcommand{\SCop}{\textsc{SC}}
\newcommand{\VLop}{\textsc{VL}}
\newcommand{\LL}{\mathit{LL}}
\newcommand{\SC}{\mathit{SC}}
\newcommand{\VL}{\mathit{VL}}
\newcommand{\sucSet}{\mathcal{S}}


\newcommand{\natType}{\mathbb{N}}
\newcommand{\boolType}{\mathbb{B}}
\newcommand{\true}{\mathtt{true}}
\newcommand{\false}{\mathtt{false}}
\newcommand{\arrayType}[2]{\mathbf{array}[#1]\ \mathbf{of}\ #2}
\newcommand{\pointerType}[1]{\mathbf{ptr}\ \mathbf{of}\ #1}
\newcommand{\NULL}{\mathtt{NULL}}
\newcommand{\valType}{\mathsf{val}}
\newcommand{\PID}{\mathtt{PID}}
\newcommand{\resX}{\mathtt{X}}
\newcommand{\resY}{\mathtt{Y}}
\newcommand{\resA}{\mathtt{A}}
\newcommand{\resB}{\mathtt{B}}
\newcommand{\resBs}{\vrt{\vsc}.\resB}
\newcommand{\resBcell}{\resB_{\mathtt{cell}}}
\newcommand{\resSS}{\mathtt{SS}}
\newcommand{\phase}{\mathtt{phase}}
\newcommand{\xPhase}{x.\phase}
\newcommand{\procA}{\mathsf{p}_\resA}
\newcommand{\procB}{\mathsf{p}_\resB}
\newcommand{\xA}{x.\procA}
\newcommand{\xB}{x.\procB}
\newcommand{\snapshot}{\mathtt{img}}
\newcommand{\xSnapshot}{x.\snapshot}
\newcommand{\toggle}{\mathtt{sync}}
\newcommand{\xToggle}{x.\toggle}
\newcommand{\ssSnapshot}{\mathit{ss}.\snapshot}
\newcommand{\ssToggle}{\mathit{ss}.\toggle}
\newcommand{\dataField}{\mathtt{data}}
\newcommand{\seqField}{\mathtt{ver}}
\newcommand{\viewField}{\mathtt{view}}
\newcommand{\movedVar}{\mathit{moved}}
\newcommand{\changedVar}{\mathit{changed}}

\newcommand{\resType}[2]{#1\ \mathsf{of}\ #2}

\newcommand{\events}{\mathsf{Events}}
\newcommand{\evStart}{\mathsf{start}}
\newcommand{\evEnd}{\mathsf{end}}
\newcommand{\evOp}{\mathsf{op}}
\newcommand{\evIn}{\mathsf{in}}
\newcommand{\evOut}{\mathsf{out}}
\newcommand{\evParent}{\mathsf{parent}}

\newcommand{\WrEff}{\mathbb{W}}
\newcommand{\vsc}{\sigma}
\newcommand{\Vsc}{\Sigma}

\newcommand{\SMap}[1]{\vrt{#1^{\bullet}}}


\newcommand{\wra}[1]{{#1}\hspace{-1pt}{\mathit{a}}}
\newcommand{\scr}[2]{{#1}\hspace{-1pt}{\mathit{r}_{#2}}}
\newcommand{\sca}[2]{{#1}\hspace{-1pt}{\mathit{a}_{#2}}}
\newcommand{\scb}[2]{{#1}\hspace{-1pt}{\mathit{b}_{#2}}}

\newcommand{\wrx}[1]{{#1}\hspace{-1pt}\mathit{x}}
\newcommand{\wrb}[1]{{#1}\hspace{-1pt}\mathit{b}}
\newcommand{\scon}[1]{{#1}_{\mathit{on}}}
\newcommand{\scoff}[1]{{#1}_{\mathit{off}}}

\newcommand{\wrf}[1]{{#1}\mathit{f}}
\newcommand{\wrfA}[1]{{#1}\mathit{f_1}}
\newcommand{\wrfB}[1]{{#1}\mathit{f_2}}
\newcommand{\wrfvsc}[1]{\fwdInter{#1}\vsc}
\newcommand{\wrfa}[1]{{#1}\hspace{-1pt}\mathit{\underline{a}}}
\newcommand{\wrfbA}[1]{{#1}\hspace{-1pt}\mathit{b}}
\newcommand{\wrfbB}[1]{{#1}\hspace{-1pt}\mathit{\underline{b}}}
\newcommand{\wrfxB}[1]{{#1}\hspace{-1pt}\mathit{\underline{x}}}

\newcommand{\scvA}{\mathit{sv_1}}
\newcommand{\scvB}{\mathit{sv_2}}
\newcommand{\scx}{s_\mathit{ss}}
\newcommand{\scv}{\mathit{v}}
\newcommand{\scvx}{\mathit{vx}}
\newcommand{\scvr}{\mathit{vr}}
\newcommand{\scva}{\mathit{va}}
\newcommand{\scvaA}{\mathit{v\overline{a}}}
\newcommand{\scvaB}{\mathit{v\underline{a}}}
\newcommand{\scvb}{\mathit{vb}}
\newcommand{\scvssA}{\scv_{\mathit{ss}}}
\newcommand{\scvxB}{\mathit{v\underline{x}}}
\newcommand{\scvss}{\scv_{\mathit{\underline{ss}}}}
\newcommand{\scvon}{\scv_{\mathit{on}}}
\newcommand{\scvoff}{\scv_{\mathit{off}}}
\newcommand{\scvend}{\scv_\mathit{end}}

\newcommand{\resXinit}{\resX_{\mathit{init}}}

\newcommand{\scxinit}[1]{{#1}_\mathit{init}}
\newcommand{\sconobs}[1]{{#1}_\mathit{\underline{on}}}
\newcommand{\scoffobs}[1]{{#1}_\mathit{\underline{off}}}
\newcommand{\scss}[1]{{#1}_{\mathit{\underline{ss}}}}
\newcommand{\scend}[1]{{#1}_{\mathit{end}}}

\newcommand{\wrs}[1]{{#1}\hspace{-1pt}{\mathit{s}}}
\newcommand{\scanth}[3]{{#1_{#3}}\hspace{-1pt}{\mathit{a}_{#2}}}
\newcommand{\scbnth}[3]{{#1_{#3}}\hspace{-1pt}{\mathit{b}_{#2}}}

\newcommand{\aref}[2]{\ifappendix{\ref{#1}}\else{#2}\fi}

\newcommand{\ifNotAppendix}[1]{\ifappendix{}\else{#1}\fi}

\newcommand{\apndxSS}{\aref{apx:ss2lin}{A}}

\newcommand{\apndxLemWhbIrrefl}{\aref{lem:whb-irrefl}{A.2}}
\newcommand{\apndxLemMaxcand}{\aref{lem:maxcand-populated}{A.4}}

\newcommand{\apndxFwd}{\aref{apx:fwd2ss}{B}}

\newcommand{\apndxJayI}{\aref{apx:jay1}{C}}

\newcommand{\apndxLemJayILin}{\aref{lem:jay1rblinpoint}{C.2}}
\newcommand{\apndxLemJayIObsX}{\aref{lem:jay1obsX}{C.1}}

\newcommand{\apndxMWFwd}{\aref{apx:mwfwd2fwd}{D}}

\newcommand{\apndxLemJayIILin}{\aref{lem:jay2rblinpoint}{D.2}}

\newcommand{\apndxJayIII}{\aref{apx:jay3}{E}}

\newcommand{\apndxLemJayIIISSEnd}{\aref{lem:jay3scssend}{E.2}}
\newcommand{\apndxLemJayIIILSEnd}{\aref{lem:jay3pushLSend2}{E.5}}

\newcommand{\apndxAfek}{\aref{apx:afek}{F}}


